TimeMachine: Timeline Generation for Knowledge-Base Entities

We present a method called TIMEMACHINE to generate a timeline of events and relations for entities in a knowledge base. For example for an actor, such a timeline should show the most important professional and personal milestones and relationships such as works, awards, collaborations, and family relationships. We develop three orthogonal timeline quality criteria that an ideal timeline should satisfy: (1) it shows events that are relevant to the entity; (2) it shows events that are temporally diverse, so they distribute along the time axis, avoiding visual crowding and allowing for easy user interaction, such as zooming in and out; and (3) it shows events that are content diverse, so they contain many different types of events (e.g., for an actor, it should show movies and marriages and awards, not just movies). We present an algorithm to generate such timelines for a given time period and screen size, based on submodular optimization and web-co-occurrence statistics with provable performance guarantees. A series of user studies using Mechanical Turk shows that all three quality criteria are crucial to produce quality timelines and that our algorithm significantly outperforms various baseline and state-of-the-art methods.

==> 010introduction_old.tex <==
% !TEX root = timelines-paper.tex
\enlargethispage{1\baselineskip} % needed to have contributions on pg 1

% [see paper outline for more details]
% motivation
% goal definition
% give example
% highlight challenges
% overview of paper
% contributions
% explain outline

\begin{figure*}[t]
	\centering
%	\includegraphics[width=\linewidth]{timeline_rdjr_full.png}
	% \includegraphics[width=0.8\linewidth]{timeline_rdjr_full.png}
  \includegraphics[width=0.8\linewidth]{timeline_rdjr_full_smaller.pdf}
%  \vspace{-2mm}
	\caption{An example timeline for Robert Downey Jr. (American actor) generated by our proposed approach.
	 Note that the timeline is interactive and displays
         explanations for each event on mouseover
(see Figure~\ref{fig:timeline_rdjr_zoom}).
Furthermore, it can be dynamically zoomed.
}
	\label{fig:timeline_rdjr_full}
  % \vspace{-0.5em}
\end{figure*}

% When querying an entity (such as a person or a movie) on a search
% engine, we are often overwhelmed by the volume and diversity of
% results. Often what we would like to see (especially when using a
% mobile device) is a brief summary of the most
% important facts related to this entity. In many cases, a convenient
% way to present this information is in the form of a timeline, with the
% key events arranged along the horizontal axis,


The volume and diversity of results when querying 
an entity (\eg, person or organization) on a search engine
can be overwhelming.
We argue that in many cases an overview
of the most important events in an organized and readable format
would serve users better,
ideally with interactive
features to enable further exploration.
A timeline with clickable key events arranged 
along a horizontal time axis would serve this need.

%a visualization dating back to the work of Joseph Priestley (1765) and
%William Playfair (1786) \cite{beniger1978quantitative}. 
%An example is shown in
%Figure~\ref{fig:timeline_rdjr_full}.
%(Note that the timeline is interactive, so that when the user mouses
%over an event, some text pops up to give more details. Also, the
%timeline can be adjusted dynamically.)

% Many people are interested in history and learning about other's lives and achievements.
% Current search engines and tools fail at providing good summaries of other individuals' lives.
% Often the best option the user is left is is to go to sites such as Wikipedia.org or biography.com and read through and digest long articles and make up their own mind about what the key events were.
% A standard approach to summarize history as a series of temporal events is to lay them out on a timeline.
% Timelines are usually visualized as a horizontal axis depicting time and displaying individual events along this axis based on when they occurred.
% Such a summarizing visualization is key to learning about a series of events efficiently.
% There is a clear need for timelines to become a core part of the search experience for temporal queries.

In this paper, we develop an approach called 
\systemname\
to automatically generate such
timelines.
The input is a knowledge base (KB) of time-stamped facts, such as
Freebase~\cite{Bollacker08}, 
Wikidata~\cite{Vrandecic2014},
or YAGO~\cite{suchanek2007yago}
(in this paper we use Freebase).
In addition, the user must specify
an entity of interest (\eg, a person).
% (In this paper, we focus on four kinds of entities:
% musicians, actors, politicians and athletes
% but the techniques are general.)
Finally, the user can optionally
specify a 
temporal interval of interest.
(If omitted, we can use a default interval,
such as from the person's date of birth to his or her date of death, or the
current time, whichever comes first.)

The output is a timeline such as the one shown in
Figure~\ref{fig:timeline_rdjr_full}, 
derived for the American actor Robert Downey Jr.
He is best known for his starring roles in the movies
{\em Iron Man} and {\em Avengers}, both of which are shown.
The timeline further depicts various family relationships (father
Robert Downey Sr., ex-wife Deborah Falconer and wife Susan Downey),
important acting roles for his career (the movie {\em Chaplin} and TV
show {\em Ally McBeal}), as well as 
other notable works and professional relationships. 
% \todo{(The images in the timeline come from Freebase.)
% They come from KG (some google service) and not from Freebase.
% }

The timeline is interactive in three ways.
First, when the user hovers over an
image,
we show various details, such as 
 ``Robert Downey Jr. starred in The Avengers, released on
 April 11, 2012''.
Second, the user can specify a particular
    time period, and a new timeline for that period will replace the current one.
    For example, Figure~\ref{fig:timeline_rdjr_zoom} shows the timeline
    for Robert Downey Jr. from 2007 until 2014 
    and gives an example event description.
The zoomed-in version focuses attention on more recent events,
such as his award for {\em Tropic Thunder}
and his role in the {\em Sherlock Holmes} movies.
Finally, the user can click on an entity icon, such as {\em Susan Downey},
    and a timeline for this entity will be displayed. 
    %(if enough interesting events exist for that entity). % Feedback from David: This is kind of implied.

An obvious method for generating such timelines is to select events with highest
global relevance scores (for example, according to a query log). 
%subject to not spreading over the display area. 
However, an empirical study shows that the results are far from satisfactory 
(see Section~\ref{sec:evaluation}).
We argue that high quality timelines should satisfy three orthogonal quality criteria:
%(in addition to being composed of actual correct events):
\begin{enumerate}
% 	\item 
% \kevin{I think we should drop this. It is too trivial/ obvious to be
%   worth mentioning. Also, we need to be consistent with the abstract,
%   that claims there are 3 criteria.}
% Correctness: Only display events that are actually true/correct.

	\item Relevance: Display only the most ``interesting'' or
          ``relevant'' events in an entity's    history.

	\item Temporal Diversity: Distribute events evenly along the
          temporal axis, to avoid visual crowding, and to allow easy
          interaction with the depicted events.

	\item Content Diversity: Display a diverse set of event types
(\eg, for an actor, do not only list the movies they have been in).
% Attempt to provide a diverse
%           representation of the subject's life. For example,  only
%           showing only movies an actor has appeared in is discouraged.
%   \todo{Consider swapping the two diversity categories (but then also
%   in evaluation section) to be parallel to the abstract?} 
\end{enumerate}
While the need for relevance is quite obvious, the
need for temporal diversity and content diversity is less clear.  
We present results from a series of user studies 
(in Section~\ref{sec:evaluation})
that clearly demonstrate the need for these two criteria.

\eat{  These types of interactions require an algorithmic solution that 
  quickly generates a timeline based on user input
  that shows relevant and diverse content
  within a limited amount of space.
  Previous work has introduced timeline generation from KBs 
through visualizing entity-level co-occurrence in news corpora~\cite{mazeika2011entity}, 
displaying events associated with an entity in the YAGO KB~\cite{wang2010timely} 
and generating context-aware timelines from Wikipedia~\cite{tuan2011cate},
  but has not yet considered these types of challenges
  (see Section~\ref{subsec:eval_relevance_signals} for an experimental comparison to the state of the art and Section~\ref{sec:relatedwork} for a discussion of related work).
}

Previous work has introduced timeline generation from knowledge bases %KBs
through visualizing entity-level co-occurrence in news corpora~\cite{mazeika2011entity}, 
displaying events associated with an entity in YAGO ~\cite{wang2010timely} 
and generating context-aware timelines from Wikipedia~\cite{tuan2011cate}.
However, none of them have addressed the challenges raised
by the diversity requirements and enabling user interaction. 
We propose a principled solution based on submodular optimization,
for which we both provide theoretical performance guarantees,
and show empirical evidence of significant improvement over baseline
and state-of-the-art methods.

%\safa{you must substantiate this claim.  Why is it challenging?  Also use the word algorithmically .. automatic 
%in computing is redundant since everything is automatic}Automatically
%generating high quality timelines is very challenging.

In particular,
our approach involves the following two main steps, which are sketched in Figure~\ref{fig:system_overview}.
First, given a subject entity of interest,
we generate as many candidate events as possible
by searching for neighboring entities with timestamps in the given knowledge base.
We generate candidate events for all possibly interesting subjects offline.
% (high coverage and high correctness).
Section~\ref{sec:generation} describes this first step in detail.
% (See Section~\ref{sec:generation} for details.)

Second, given a set of candidates and a time period of interest, we
select (online, or at run time)
a diverse subset of the most relevant events subject to temporal diversity or layout constraints.
% (high relevance, high content diversity, and high temporal diversity). 
% We extract the candidate events from the Freebase knowledge graph.
% Even though it is known that Freebase (and similar 
% \safa{not KB but KG .. I think it is important that this method relies on a graph and not just any Knowledge Base}KBs, such as YAGO)
% is quite incomplete (\safa{delete "in the sense that"}in the
% sense that many mandatory relations between entities are missing)
% \cite{Dong14},
% we show that we can nevertheless extract a large number of candidate
% events for a large number of popular entities.
% The details of this process are 
% described in Section~\ref{sec:generation}.
To do this, we maximize a submodular objective using various
relevance signals based on web co-occurrence, 
subject to these layout constraints.
% (which is more complex than the more standard set
%cardinality constraint).
We prove that our greedy algorithm for optimization
yields close-to-optimal solutions.
In addition, 
our algorithm allows for fast dynamic updates of the timeline based on
user interaction (zooming in or out).
%We choose this two-step approach to enable fast timeline generation for user-defined time spans.
% and for different form factors (e.g. desktop vs mobile).
% (See Section~\ref{sec:selection} for details.)
Section~\ref{sec:selection} describes this second step in detail.

% Kevin added this, just because we have already discussed sec 2-3
% so it feels odd to not discuss the remaining sections
Section~\ref{sec:evaluation} evaluates our proposed algorithm and
compares it to various simpler
baselines and current approaches. Section~\ref{sec:relatedwork} summarizes related work,
Section~\ref{sec:future} discusses future work,
and finally Section~\ref{sec:conclusion} concludes.


%The objective function contains various terms that measure the
%relevance of candidate entitites.
%We propose different relevance signals, based on
%entity-entity and entity-date co-occurrence statistics derived from a large web corpus.
% We present a comprehensive evaluation of our system and the relative
% importance of different parts through a series of large-scale user
% studies on Amazon Mechanical Turk.
% This is described in Section~\ref{sec:evaluation}.

In summary, our main contributions are as follows.
\begin{enumerate}
%interactive timeline search
  \item A design of a timeline search engine that efficiently 
        supports various types of user interaction.
  % \item A design of a timeline search system that allows for 
  %       efficient dynamic modification of timelines 
  %       based on user interaction.

	\item An algorithm for generating entity
          timelines based on submodular optimization
          and web-co-occurrence scores.

% 	\item An efficient way to dynamically modify timelines
% based on user interaction.

	\item An extensive user study of the relative importance of
          different signals for determining entity relevance
          and different notions of diversity.
\end{enumerate}
\vspace{-1.0\baselineskip}

% The remainder of the paper is organized as follows: 
% Section~\ref{sec:generation} details the event candidate generation phase and the second phase, event selection, is described in Section~\ref{sec:selection}. 
% Experimental results are presented in Section~\ref{sec:evaluation}.
% We discuss related work in Section in Section~\ref{sec:relatedwork} before we conclude the paper in Section~\ref{sec:conclusion}.


\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{system_architecture_new_black_newfont.pdf}
%  \vspace{-5mm}
	\caption{System architecture.
{\sc TimeMachine} traverses the KB offline to generate candidate events for 
a subject of interest (\eg, {\em Robert Downey Jr}, represented by Freebase ID {\em /m/016z2j}).
At run time, the user specifies a time period (\eg, {\em 1988--2014}) of interest,
and {\sc TimeMachine} selects a subset of events from the candidates to generate the timeline.
}
	\label{fig:system_overview}
  % \vspace{-0.5em}
\end{figure}




==> 015problem.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{timeline_rdjr_zoom.png}
%   \caption{An example timeline for Robert Downey Jr,
% where we have zoomed in on the most recent years of his life.
% }
%   \label{fig:timeline_rdjr_zoom}
%   % \vspace{-0.5em}
% \end{figure*}

\smallskip
\noindent
{\bf System design:}
We envision a system called {\sc AboutTime} to support search for the timeline of important events
related to a particular subject. For this paper we assume both the subject and the events on
the timeline come from a {\em knowledge base (KB)}, such as {\em Freebase}~\cite{freebase}.
The KB contains a set of {\tt (subject, predicate, object)} triples
in the RDF format. We leave the problem of history extraction 
from the Web for future research.

When a user specifies a subject such as 
{\em Robert Downey Jr.}, {\sc AboutTime} would show a timeline as in 
Figure~\ref{fig:timeline_rdjr_full} for his life period (\ie, from his birth date 
to his death date or ``now''). 
The timeline consists of a set of {\em events}, each associated with a representing
entity and a timestamp. For each entity the timeline shows a picture icon 
of a fixed width and height; how to select the picture is orthogonal to our problem
and in practice we use the picture specified in {\em Freebase}. 
The picture icons should never overlap; one may stack on top of another if needed.
\eat{For simplicity we use a layout strategy called {\em Order-Layout}, where we 
(1) order the entities by their time stamp, 
(2) put each entity on the timeline according to its timestamp, 
and (3) stack one entity on top of another if putting them on the
same layer would overlap the icons.}
The timeline allows three types of interactions.
\begin{itemize}
  \item {\em Showing details:} When a user hovers the mouse over an entity icon,
    such as {\em The Avengers}, details will be displayed for the event such as 
    {\em ``Robert Downey Jr. starred in The Avenger, released on 2012/04/11''.}
  \item {\em Zooming in and out:} The user can slide the time bar to specify a particular
    time period, and a new timeline for that period will replace the current one.
    For example, Figure~\ref{fig:timeline_rdjr_zoom} shows the timeline
    for {\em Robert Downey Jr.} from 2007 up to now.
  \item {\em Jumping to another entity:} The user can click on an entity icon, such as {\em Susan Downey},
    and a timeline for this entity will be displayed if that entity also has a ``history''.
\end{itemize}

\smallskip
\noindent
{\bf Problem definition:}
The core problem to support timeline search is to generate a timeline for a given subject
and a given time period, fitting in a particular screen area with a given width and height. 
We formally define the problem as follows.

\begin{definition}[Timeline Generation]
Let $\cal K$ be a knowledge base and $\tt s$ be a subject in $\cal K$.
Let $[T_1, T_2]$ be a time period. Let $W$ and $H$ be the width and height
of a screen box, and $w$ and $h$ be the width and height of
a picture icon. The {\em Timeline Generation} problem generates
a timeline with a set $\bf E$ of events such that
\begin{itemize}
  \item each event $e \in \bf E$ represents a historical event for $\tt s$,
    is associated with a representing entity (maybe $\tt s$ itself) in $\cal K$,
    and happens at time $t({\tt s}, e) \in [T_1, T_2]$;
  \item the picture icons of size $h$x$w$ for events in $\bf E$ can fit in the screen of size $H$x$W$.
\end{itemize}
\end{definition}

Note that this definition skips three pieces of details.
The first is about which event represents a historical event for $\tt s$.
In general it should happen at a particular time in a person's life 
and Section~\ref{subsec:event_generation} gives our criteria.
The second is about how the picture icons can fit in a screen. This depends on the strategy
we lay out the icons and Section~\ref{subsec:temporal_constraint} discusses the details.
The third is about which set of events form the best timeline. In general 
we have three requirements and Section~\ref{subsubsec:entity_relevance} gives the formal metric.
\begin{itemize}
  \item {\em Relevance:} event $e \in \bf E$ should be highly relevant to $\tt s$ 
    in search and in Web articles.
  \item {\em Content diversity:} the events in $\bf E$ should have different
    types (\eg, publishing an album vs. starring in a movie).
  \item {\em Temporal diversity:} the events in $\bf E$ are fairly evenly
    distributed along the timeline.
\end{itemize}

\smallskip
\noindent
{\bf Architecture and overview:}
Figure~\ref{fig:system_overview} depicts the architecture for timeline generation. 
We solve the problem in two steps. First, at offline time
the {\em Candidate Event Generation} component takes the KB 
and a subject as input, identifies the set of all historical events 
from the KB; for each event, it generates the representing entity and
a timestamp. The results should have high {\em correctness} and {\em coverage}.
Section~\ref{sec:generation} describes how we traverse the knowledge base 
for candidate generation. To obtain a high coverage, we consider not only
direct relationship such as {\em Robert Downey Jr. stared in movie 
The Avengers}, but also indirect relationship such as {\em Robert Downey
Jr. and Chris Evans co-star in The Avengers} (Section~\ref{subsec:event_generation}). 
To obtain a high correctness, we filter paths that are over-common in the KB 
or violate certain constraints (Section~\ref{subsec:event_filtering}). 

Second, the {\em Event Selection} component takes as input a particular
time period at runtime,  selects from the candidates a set of events to construct the timeline.
The selected events should be {\em relevant, diverse}, and satisfy
the layout constraint. Section~\ref{sec:selection} formalizes the problem
as an optimization problem, where the objective function captures the
relevance and diversity, and the constraint captures the layout restriction
(Section~\ref{subsec:timeline_optimization}). It then proves that the objective
function is {\em submodular} and the constraint forms an {\em independence family}
(we give the definition later), leading to a greedy algorithm with an approximation
guarantee (Section~\ref{subsec:optimization_algorithm}).




==> 040evaluation_old.tex <==
% !TEX root = timelines-paper.tex

\todo{I probably jump in verb tense a lot. Check and unify.}
\todo{stress more that we perform qualitative evaluation (see examples and demo, maybe talk about RDJr improvements)}
\todo{stress that we have quantitative evaluation through user study}


This section presents the evaluation of our proposed approach to generate timelines through a series of user studies.
Qualitative examples were shown in Figure~\ref{fig:timeline_rdjr_full} and Figure~\ref{fig:timeline_rdjr_zoom} (zoom).
For more examples, try out our demo\footnote{\label{footnote:demo}\url{http://cs.stanford.edu/~althoff/timelines} (user ``timelines'', password ``84orangehorses'')}.

We investigate the importance of the three\todo{?} quality criteria introduced in Section~\ref{sec:introduction}: Relevance, Temporal Diversity, and Content Diversity.
Since there is are ground truth timeline datasets available we evaluate the relative importance of each of the three quality criteria through a series of user studies on Amazon Mechanical Turk \todo{citation needed}.


\subsection{User Study Instructions}
\label{subsec:user_study_instructions}
Initial user studies showed that evaluating timelines can be challenging and require some domain knowledge.
In particular, raters were often overwhelmed when asked to consider multiple criteria at the same time or when they were not familiar with the timeline subject.
To address these challenges, we ask raters
(1) for relative judgments between two timelines generated by similar approaches so that they can focus on a limited number of differences (we randomize the order of the two timelines shown), 
(2) to only focus and judge one criterion at a time (we control the other two criteria), and 
(3) we largely use head entities that raters would be more likely to be familiar with and ask them to first familiarize themselves with the entity in question by reading the corresponding Wikipedia article and perform searches as needed.
We also ask them to carefully consider all events in the timelines and their respective descriptions (see Section~\ref{subsec:experimental_setup} and Figure~\ref{fig:timeline_rdjr_zoom}).

In addition to the relative judgment for each timeline pair, raters are asked to explain their decision in a few sentences and highlight important differences between the two timelines.
Example explanation of a rating of Robert Downey Jr's timeline (rejecting \textsc{G2E+E2D} in favor of the proposed approach): ``Bottom time line does not include any reference to iron man. Iron man catapulted his comeback in the film industry and should definitely been included in his timeline.''
% There are longer and more expert-like quotes but I think it's good to go with RDJr again.
We also provided a multiple-choice list of major failure cases: 
``Too many repetitions of the same types of events or explanations'', 
``Some descriptions are confusing'', 
``Timelines are identical'', 
``Other reasons'').



\subsection{Baseline}
\label{subsec:baseline}
We compare our approach to a baseline that uses a static global signal (\GtoE~as described in Section~\ref{subsubsec:entity_relevance}) without any reranking or dynamic updates based on temporal or content diversity.
Early user studies showed very negative reactions to bad layout or insufficient content diversity which lead us to explicitly model these criteria and consider user studies that test the three criteria separately.
Otherwise, failures in temporal or content diversity would almost always trump differences in relevance signals requiring explicit control of diversity.
We also found the increased focus to yield more useful and less noisy ratings.

Since the \GtoE~baseline was outperformed so strongly in initial studies, we augment it by enforcing temporal diversity as well as a hard content diversity constraint (do not show the same related entity more than once).
We show below that this augmented baseline (referred to as \textsc{G2E+Div}) is still significantly outperformed by our proposed approach.



\subsection{Experimental Setup}
\label{subsec:experimental_setup}
For the event generation phase (see Section~\ref{sec:generation}) we use the public knowledge base Freebase \cite{Bollacker08}.
While Freebase is known to be incomplete \todo{citation needed} the proposed approach still obtains high coverage (recall Figure~\ref{fig:path_coverage}).

As discussed in Section~\ref{subsec:zoom}, our approach allows for different form factors and can optimally select events for both mobile and desktop environments.
For the evaluation, we only focus on desktop environments and use a height of $n=2$ (1000px width).

Through a number of initial user studies we learned that users tend to prefer the \entityrelevance~signal over the \daterelevance~signal.
Therefore, we emphasize the \entityrelevance~signal in our ``full'' approach \textsc{G2E+E2E+E2D} ($\lambda=0.75$, $w^e_1 = w^d_1 = 1$, $w^e_2 = w^d_2 = 10^{-2}$, and $w^e_3= 10^{-4}$).
This set of parameters is used for all experiments unless noted otherwise.
Note that we use plus signs (+) to indicate addition of signals or components and and use minus signs (-) to indicate removal of signals or components.

To allow users in our user study to understand, differentiate, and judge timeline events it is necessary to explain the events and relationships in natural language (instead of abstract paths over KB predicates).
To this end, we generate English descriptions for each KB path and display them when the user hovers over the event (see Figure \todo{Illustrate hover explanation in zoomed in example} or our interactive demo\footnotemark[\value{footnote}]). %\footnotemark[\ref{footnote:demo}]
We achieve this through a manual mapping of paths to simple patterns such as ``$\sub$ married $re_1$ on $t$.'' for the most frequently occurring 100 paths.
For rare paths we fall back to the English names for the individual predicates in the path which yields understandable but grammatically incorrect descriptions of the relationship captured by the path.




\subsubsection{Evaluation Metrics}
\label{subsubsec:evaluation_metrics}

Each experiment corresponds to a pairwise comparison between two event selection methods for a fixed set of timeline subjects.
Each comparison (method A vs method B on entity \sub) is replicated five times and sent to different raters.
Ratings were collected on a 5 point scale even though we only consider 3 levels, preferring A, tie, or preferring B (initial experiments showed that a 5 point scale yields best ratings even if one is only interested in binary judgments).

We report two orthogonal metrics: rater agreement (how much do raters agree on which timeline is better?), and rater preference (how much do raters prefer one method over the other)?
Rater agreement (RAggr) is measured as the fraction of agreeing pairs of ratings for each entity (e.g. 3A vs 2B would lead to 40\% agreement).
Rater preference (RPref) is calculated by
first aggregating the ratings for each entity and then casting a vote if there is a majority for either A, tie, or B.
Ignoring ties, we compute the fraction of times method A was the majority preference.
If both methods were equally good one would expect a fraction of 50\%. 
We use exact, two-sided binomial tests to measure statistical significance of our results ($H_0: p=0.5)$.

\todo{should we include any other information from the table in \url{https://docs.google.com/spreadsheets/d/146BoTVZdh-h-p_vbfurJvGvJ1Srk3h4el08N8C8Wr7s/edit#gid=0}? e.g. results on rating level or kappa?}


\subsubsection{Experiments}
\label{subsubsec:experiments}
We designed a series of experiments to answer the following questions and shine a light on their relative importance for timeline generation.
Every experiment corresponds to a pairwise comparison between two different timelines selection approaches.
We use a set of 250 popular entities (75 music artists \& bands, 75 actors, 50 politicians, 50 athletes).
Most raters reported to already be familiar with these entities (79\%).
Each pair of timelines is rated by five different raters (1154 distinct raters total).

\xhdr{Relevance} \textit{What relevance signals in event selection are most appreciated by users?}\\
We compare the full approach \textsc{G2E+E2E+E2D} (referred to as \textsc{Full}) to a version without the \EtoD~signal (\textsc{G2E+E2E}; $\lambda=1$), 
a version without \EtoE~signal (\textsc{G2E+E2D}; $w_1^e = w_2^e = 0$), 
\todo{$\lambda=0$ is actually incorrect since it zeroes out G2E.}
and the augmented baseline (\textsc{G2E+Div}; $\lambda = w_3^e = 1$, $w_1^e = w_2^e = 0$; as described in Section~\ref{subsec:baseline}).

\xhdr{Temporal Diversity}: \textit{Do users appreciate having a constrained layout the never overpopulates parts of the timeline?}\\
We compare the full approach \textsc{Full} to a version that does not consider the temporal diversity constraint \textsc{Full-TempDiv} (see Section~\ref{subsec:temporal_constraint}).
More specifically, this version selects the same number of events as the full approach without consideration of the layout constraint, i.e. solving the optimization problem in Equation~\eqref{eq:timeline_optimization} with a simple cardinality constraint instead of \temporalconstraints.
We then remove overlapping event boxes (removing the less relevant event) in the visualization since that causes raters to rate this version worse as shown by previous user studies.
\todo{Should we note that this can be achieved by simply rerunning the optimization with temporal constraints on the candidate set that is the output of the previous ``unconstrained'' run?}
Since this effect was found to be very strong in early studies across a diverse set of entities we use a smaller set of 30 entities for this experiment. 

\xhdr{Content Diversity} \textit{Do users appreciate more diverse events potentially at the expense of relevance?}\\
We compare two different versions of content diversity, hard constraints (strictly permit any duplicate related entities; used in \textsc{Full} approach in previous experiments to ensure that they are not impacted by differences in content diversity), and soft constraints\linebreak[4] \textsc{Full+Soft} using the weighted coverage functions as described in Section~\ref{subsubsec:entity_relevance}
to a version that does not encourage content diversity \textsc{Full-ContDiv}.
In this version, we replace the coverage functions \EtoE, \EtoEPath, and \GtoE~by simple sums over all entities in the timeline (i.e. a sum over a multiset of related entities), including duplicate related entities, and give the full ``reward'' each time.
In contrast, coverage functions are functions over the set of related entities (without duplicates) that only reward one occurrence and thereby encourage diversity).



\subsection{Experimental Results \& Discussion}
\label{subsec:experimental_results}

\newcommand{\signone}{\textsuperscript{}}
\newcommand{\sigone}{\textsuperscript{*}}
\newcommand{\sigtwo}{\textsuperscript{**}}
\newcommand{\sigthree}{\textsuperscript{***}}

\begin{table}[t]
\small
% \fontsize{6}{7.2}\selectfont
\begin{center}
%\setlength{\tabcolsep}{6pt}
\begin{tabular}{p{0.2\columnwidth} p{0.3\columnwidth} r r r@{}l } % p{0.2\columnwidth} %@{\hspace{6pt}} 
\toprule
\textbf{Method A} & \textbf{Method B} & \textbf{\#Raters} & \textbf{RAggr} & \multicolumn{2}{c}{\textbf{RPref}} \\
\midrule
\textsc{Full} & \textsc{G2E+Div} & 344 & 61.8 & 83.8 & \sigthree \\
\textsc{Full} & \textsc{G2E+E2E} & 463 & 60.0 & 59.8 & \sigtwo \\
\textsc{Full} & \textsc{G2E+E2D} & 676 & 56.6 & 64.4 & \sigthree \\
\sectionrule
% \midrule
\textsc{Full} & \textsc{Full-TempDiv} & 53 & 59.3 & 86.7 & \sigthree \\
\sectionrule
% \midrule
\textsc{Full} & \textsc{Full-ContDiv} & 665 & 68.1 & 91.1 & \sigthree \\
\textsc{Full+Soft} & \textsc{Full-ContDiv} & 677 & 68.6 & 90.3 & \sigthree \\
\bottomrule
\sectionrule
\multicolumn{4}{l}{\scriptsize{\textsuperscript{***}$p<0.001$, 
  \textsuperscript{**}$p<0.01$, 
  \textsuperscript{*}$p<0.05$}}
\end{tabular}
% \vspace{-1mm}
\caption{Summary statistics for a series of user studies that each correspond to a pairwise comparison between to different event selection approaches. We report the number of distinct raters that partook in each study, the fraction of agreeing rating pairs (RAggr), as well as the fraction of entities for which raters strictly prefer method A over method B (RPref).
\todo{fix font sizes and presentation somehow. We could add number of entities, ties, and eval on rating level and make it a double column table}. Make last column bold?}
\label{table:evaluation_results}
% \vspace{-3mm}
\end{center}
\end{table}


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{results_with_conf_int.pdf}
  \caption{Median fraction of entities for which raters preferred method A (first) over method B (second) along with bootstrapped confidence intervals. 
  Raters significantly preferred the proposed approach in all cases.
  \todo{TIM: update figure with new labels.}}
  \label{fig:results_with_ci}
  % \vspace{-0.5em}
\end{figure}

% Tim: I merged results & discussion. Thoughts?
% \subsection{Discussion}
% \label{subsec:discussion}

The experimental results are summarized in Table~\ref{table:evaluation_results}.
Figure~\ref{fig:results_with_ci} shows the fraction of preference for our proposed approach along with bootstrapped confidence intervals.
All differences are statistically significant according to two-sided Binomial tests ($p\ll0.001$; \textsc{G2E+E2E}: $p<0.01$)

The augmented baseline \textsc{G2E+Div} is rejected in favor of our proposed approach in over 83\% of all cases.
This demonstrates that a global importance measure, even in the presence of temporal and content diversity, is clearly insufficient.
The \EtoE~signal is most strongly correlated with user preferences among the three individual signals. 
However, in 60\% of all cases users strictly preferred the full approach over \textsc{G2E+E2E}.
The \EtoD~signal performs quite well by itself, users prefer the full approach in 64\% of all cases.

% should this section with more detailed information about E2E and E2D go somewhere else?
% E2D works best for music artist -> Which events does E2D favor?
% E2E favors what? -> check additional doc
Analyzing the the verticals (music artists, actors, politicians, athletes) individually we found that the \EtoE~signal was more important for actors and athletes and that music artists benefited most from the \EtoD~signal.
Since both signals are based on web co-occurrence they both depend on entity/entity or entity/date co-mentions that are subject to certain conventions on the web.
We found this to be particularly for dates: many articles list date of birth/death, marriage explicitely and be much more vague about the exact time of other events.
For musicians, it is common to mention the date when an album was released (e.g. on semi-structured web-pages like online stores).
It is less common to directly associate e.g. a movie release date with a particular actor and when it is done often only very few star actors are mentioned in these promotional articles.
Restricting oneself to the \EtoD~signal only one also looses the ability to properly distinguish between events with the same timestamp, i.e. should one prefer to show the movie itself, other actors, or the producer at the movie release date?
We further found that the \EtoD~signal has less utility when events do no not exhibit a clear temporal focus such as long military conflicts (compared to birth/death/marriage dates or concert tours).
In these cases, the \EtoE is helpful in providing additional information in the event selection phase.


Users disliked cluttered and unbalanced very strongly in our experiments and prefer the enforcement of temporal diversity constraints (as described in Section~\ref{subsec:temporal_constraint}) 87\% of the time. 

We found equally strong effects when we did not encourage content diversity -- users preferred more diverse timelines over 90\% of the time.
In over 70\% of all cases, the rejected baseline was found to be ``too repetive'', compared to only 12\% for the proposed approach.

Over 70\% of ratings give ``too repetitive'' as a reason for rejecting the less diverse option compared to 12\% when rejecting the proposed approach. 
However, the reason ``irrelevant events'' increases slightly illustrating the trade-off between showing more diverse results and making more mistakes by taking this risk.
It did not matter whether this content diversity was enforced as a constraint (\textsc{Full}) or merely encouraged through diminishing returns as modeled in the submodular objective (\textsc{Full+Soft}).
This means that it is not necessary to add a manual hard constraint in addition to our less strict submodular objective.

Analyzing the ratings for temporal and content separately for each vertical we found that the effect was consistent and significant across all verticals.

We conclude that if one is restricted to a single signal one should go with the \EtoE~signal but that there is significant value in combining \EtoE~and \EtoD~signals.
Using a global static ranking of entity relevance is demonstrated to be insufficient.
We find that it is absolutely crucial to encourage both temporal and content diversity.





\subsection{Error Analysis} % Or conceptual limitations (and failure cases)
\label{subsec:error_analysis}
This section discusses the main error sources identified throughout the series of user studies.

\xhdr{Presentation}
Deciding which time period (or cluster of events) to show is a challenging problem in itself.
For many entities, the most important events happened during a short period of their life.
Therefore, we addressed this challenge by choosing the shortest time period that covers at least 90\% of all generated events (restricted to their lifetime if the timeline entity is a person).
One instance where this failed was for US president John F Kennedy for whom many important events occurred in the last few years of his life (assassination, presidency, Cuban missile crisis, Bay of Pigs invasion etc.).
Because of the algorithm by default attempts to cover 90\% of all generated events the timeline can only contain very few events from this short but important period.
In our concrete case, assassination, presidency, and his marriage to Jacqueline Kennedy Onassis are chosen first and then block other important events such as Cuban Missile Crisis or his involvement in the Vietnam war.
However, this can clearly be improved e.g. (1) by using \EtoD~scores to weight some time periods more important than others or (2) by including the search over suitable time periods as part of the the optimization problem.
Note however, that simply zooming into this period of his life quickly resolves the issue as well.


\xhdr{Representation}
We assume a very simple but flexible format of events (see Section~\ref{sec:generation}) that considers subject, related entity, timestamp and the paths connecting them.
In the vast majority of cases this simple framework encodes all the infqormation necessary.
However, it turns out that in Freebase some CVT nodes (see Section~\ref{sec:CVT}) \todo{Section got removed} are qualified by additional attributes that can be important.
For example the \texttt{/people/marriage/from} is not only used for marriages but also for domestic partnerships (and ignoring this qualification would result in false inferences).
We also found that users reported certain types of events to be confusing, for instance using the date of death as the date that the marriage ended, or describing US presidents as military commanders.
While the President of America is also the Chief of the Armed Forces, a president is never really thought of as a military commander giving military orders, but as a politician.
Additional filters might be necessary to deal with these cases where the powerful representation in knowledge bases can overwhelm the user.
We also note that our event representation only allows for a single timestamp and thus does not capture time periods. 
In this framework, start and end are simply treated as two events and often the algorithm chooses one or the other depending on temporal constraints.
However, our approach could be extended to allow for time periods as well (though the visualization of time periods might impact the formulation of the temporal constraint).


\xhdr{User Preferences \& Personalization}
Users have different preferences and opinions and timelines are not at all exempt to these.
The closer the presented two timelines are in terms of objective quality the easier you can observe when people simply have different opinions rather than all converging to the same objective answer.
Therefore, rater agreement (RAggr) will never be perfect unless there is such a big difference in objective quality that trumps any other personal preferences.
In our experiments, the biggest area of disagreement is over how much the timeline should be focused on professional life (e.g. created artifacts) and personal life and relationships (marriage, children etc).
Users had different opinions, even for the exact same timeline entities, which illustrates the need for personalization in this space.
This also leads to the question whether we should conceptually distinguish between artifacts (e.g. movies, albums, bills, books, military conflicts) and connections (e.g. people, relationships) and plan to investigate this matter in future work.
This would allow for controlled variation in professional vs. personal life events subject to personal preferences.


\xhdr{Extractive vs Abstractive Summarization}
The event selection phase can be viewed as a lifetime summarization task similar to text summarization.
Such tasks are commonly formulated as a selection problem (\todo{do we know of notable examples or exceptions?}) and conceptually belong to the category of extractive summarization methods.
In contrast, abstractive summarization methods build an internal semantic representation and then use natural language generation techniques to create a summary.
Most research, including ours, has focused primarily on extractive methods. 
However, we believe that abstractive techniques could be particularly useful for summarization tasks based on knowledge bases since an internal semantic representation is readily available.
Since our proposed framework subscribes to the extractive approach, the algorithm may be forced to select a single event to describe a multi-faceted relationship.
In the case of Robert Downey Jr, a user noted ``The bottom [timeline] includes more movies, plus includes his father (although the description for his father is weirdly specific).''
His father is also a filmmaker and Robert Downey Jr has starred in one of his father's movies (which is depicted by the event).



